Learning Object-Based State Estimators for Household Robots

A robot operating in a household makes observations of multiple objects as it moves around over the course of days or weeks. The objects may be moved by inhabitants, but not completely at random. The robot may be called upon later to retrieve objects and will need a long-term object-based memory in order to know how to find them. Existing work in semantic slam does not attempt to capture the dynamics of object movement. In this paper, we combine some aspects of classic techniques for data-association filtering with modern attention-based neural networks to construct object-based memory systems that operate on high-dimensional observations and hypotheses. We perform end-to-end learning on labeled observation trajectories to learn both the transition and observation models. We demonstrate the system's effectiveness in maintaining memory of dynamically changing objects in both simulated environment and real images, and demonstrate improvements over classical structured approaches as well as unstructured neural approaches. Additional information available at project website: https://yilundu.github.io/obm/.

==> figText/ablations.tex <==
\begin{table}[t]
\footnotesize
\centering
\scalebox{0.8}{
\setlength{\tabcolsep}{2.5pt}
\centering
\begin{tabular}{c|c|c|c|cccc}
    \toprule
    Sparsity &  Learned & Suppression  & Relevance & \multicolumn{4}{c}{Observations} \\
     & Memory  & & & & & \\
    \midrule
    & & & & 10 & 30 & 50 & 100\\ 
    \midrule
     \textbf{-} &  \textbf{--} &  \textbf{--}&   \textbf{--}& 0.382 & 0.452 & 0.474 & 0.487   \\\
     \textbf{+} &  \textbf{--} &  \textbf{--} &  \textbf{--} & 0.384 & 0.412 & 0.423 & 0.430 \\\
     \textbf{+} & \textbf{+} & \textbf{--} & \textbf{--}  & 0.335  & 0.357 & 0.366  & 0.387  \\
    \textbf{+} & \textbf{+} & \textbf{+} & \textbf{--}  &  0.279 & 0.274 & 0.278 & 0.282 \\
    \textbf{+} & \textbf{+} &  \textbf{+} &  \textbf{+} & \textbf{0.238} & \textbf{0.157} & \textbf{0.137} & \textbf{0.131}\\
    \bottomrule
\end{tabular}
}
\caption{\small \textbf{Ablation Analysis.} We ablate each component of \model on the {\em Normal} distribution . When learned memory is ablated, \model updates states based on observed values (appropriate in the {\em Normal} distribution dataset).}
\label{tbl:ablations}
\end{table}

==> figText/cluster_infer.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{fig/components_infer.pdf}
\caption{\small \textbf{Generalization to Increased Cluster Number.} Plots of inferred number of components using a confidence threshold in \model compared to the ground truth number of clusters (\model is trained on only 3 clusters). We consider two scenarios, a noisy scenario where cluster centers are randomly drawn from -1 to 1 (left) and a scenario where all added cluster components are well seperated from each other (right). \model is able to infer more clusters in both scenarios, with better performance when cluster centers are more distinct from each other.} 
\label{fig:cluster_infer}
\end{figure}

==> figText/cluster_more.tex <==
\begin{table}
\footnotesize
\setlength{\tabcolsep}{5.5pt}
\centering
\scalebox{0.8}{
\begin{tabular}{l|c|ccccc}
    \toprule
   Model & Online &  \multicolumn{4}{c}{Observations} \\
    \midrule
    & & 50  & 65 & 80 & 100 \\
      \midrule
    \model &  \textbf{+} & \textbf{0.158} & \textbf{0.154} & \textbf{0.151} & \textbf{0.147}\\
     VQ  & \textbf{+}  & 0.162  & 0.157  & 0.153  & 0.148 \\
    \midrule
     K-means++ & \textbf{-} & \textbf{0.155} & \textbf{0.151}  & \textbf{0.148 } & \textbf{0.146 } \\
     GMM & \textbf{-} & 0.156  & 0.151  & 0.149  & 0.147 \\
    \bottomrule
\end{tabular}
}
\caption{\small \textbf{Performance on Large Number of Clusters.} Comparison of performance on {\em Normal} distribution, when underlying distributions have a large number of components. We use 30 components, and train models with 50 observations. Each cluster observation and center is drawn between -1 and 1, with reported error as the L2 distance between predicted and ground truth means.}
\label{tbl:cluster_more}
\vspace{-10pt}
\end{table}

==> figText/cluster_num.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{fig/obs_gen.pdf}
    \vspace{-10pt}
    \caption{\small \textbf{Generalization with Increased Observations.} Plot of LSTM, Set Transformer and \model errors when executed {\em at test time} on different number of observations from the {\em Normal} distribution. With increased observations, \model error continues to decrease while other approaches obtain higher error.}
    \label{fig:gen}
    \vspace{-20pt}
\end{figure}








==> figText/comparison_distribution.tex <==
\begin{table}
\footnotesize
\setlength{\tabcolsep}{5.5pt}
\centering
\scalebox{0.8}{
\begin{tabular}{l|c|c|ccccc}
    \toprule
     Model & Online & Learned & Normal & Elongated & Mixed & Angular & Noise \\
     \midrule
     \model &  \textbf{+} & \textbf{+} & \textbf{0.157} & \textbf{0.191} & \textbf{0.184} &  \textbf{0.794} & \textbf{0.343}\\
     Set Transformer  & \textbf{+} & \textbf{+} & 0.407  & 0.395  & 0.384 & 0.794  & 0.424  \\
     LSTM & \textbf{+} & \textbf{+} &  0.256  & 0.272 & 0.274  &  0.799  & 0.408 \\
     VQ  & \textbf{+} & \textbf{-} &  0.173  & 0.195 & 0.191 & 0.992 & 0.947 \\
     \midrule
     Set Transformer & \textbf{-} & \textbf{+} &  0.226 & 0.248 & 0.274 & \textbf{0.816} & \textbf{0.406} \\
     Slot Attention  & \textbf{-} & \textbf{-} &  0.254  & 0.267 & 0.268 & 0.823 & 0.504 \\
     K-means++ & \textbf{-} & \textbf{-} &  \textbf{0.103} & \textbf{0.139} & \textbf{0.135} & 0.822  & 1.259 \\
     GMM & \textbf{-} & \textbf{-} &  0.113  & 0.141  & 0.136  & 0.865  & 1.207  \\
        \bottomrule
\end{tabular}
}
\caption{\small \textbf{Quantitative Results on Online Clustering.} Comparison of performance on clustering performance across different distributions. Reported error is the L2 distance between predicted and ground truth means. Methods in the bottom half of table operate on observations in bulk and thus are not directly comparable. 
}
\label{tbl:comparisons-dist}
\vspace{-15pt}
\end{table}

==> figText/comparison_images.tex <==
\begin{table}
\footnotesize
\centering
\scalebox{0.8}{
\setlength{\tabcolsep}{2.5pt}
\centering
\begin{tabular}{l|c|cccc|cccc}
    \toprule
    Model & Learned & \multicolumn{4}{c|}{MNIST} & \multicolumn{4}{c}{Airplanes} \\
    \midrule
     Observations &  & 10 & 30 & 50  & 100 & 10 & 30 & 50 & 100 \\
     \midrule
    \model & \textbf{+} & 
    \textbf{7.143} & \textbf{5.593} & \textbf{5.504} & \textbf{5.580} & \textbf{4.558} & \textbf{4.337} & \textbf{4.331} & \textbf{4.325} \\
     LSTM & \textbf{+} & 9.980  & 9.208  & 9.166  & 9.267  & 5.106  & 4.992  & 4.983  & 4.998   \\
    K-means  & \textbf{+} & 13.596  & 12.505 & 12.261 & 12.021 & 7.246 & 6.943  & 6.878 & 6.815 \\
    \bottomrule
\end{tabular}
}
\caption{\small \textbf{Quantitative Results on Image Domain.} Comparison of entity-monitoring performance  on MNIST and Airplane datasets across 10, 30, 50, 100 observations. For \model, LSTM and K-means we use a convolutional encoder/decoder trained on the data.  We train models with 30 observations and report MSE error.}
\label{tbl:comparison_images}
\vspace{-5pt}
\end{table}


==> figText/comparisons_dynamic.tex <==

\begin{table}[t]
\footnotesize
\setlength{\tabcolsep}{5.5pt}
\centering
\scalebox{0.8}{
\begin{tabular}{l|cccc}
    \toprule
  Model &  \multicolumn{4}{c}{Observations} \\
    \midrule
    &  10 & 20 & 30  & 40 \\
      \midrule
    \model & \textbf{0.415} & 0.395 & 0.382 & 0.394 \\
     Set Transformer  & 0.699 & 0.701 & 0.854 & 1.007    \\
     LSTM  &  0.422 & 0.400 & 0.445 & 0.464 \\
     \midrule
     JPDA (oracle) & 0.683 &  \textbf{0.372} & \textbf{0.362} & \textbf{0.322}\\
        \bottomrule
\end{tabular}
}
\caption{\small \textbf{Performance on Dynamic Objects.} Comparison of different methods on estimating the state of 3 dynamically moving objects.  All learning models are trained with 1000 sequences of 30 observations. We report MSE error. JPDA uses the ground-truth observation and dynamics models.}
\label{tbl:comparisons-dynamic}
\vspace{-15pt}
\end{table}

==> figText/comparisons_normal.tex <==
\begin{table}[t]
\footnotesize
\setlength{\tabcolsep}{5.5pt}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|c|c|ccccc}
    \toprule
   Model & Online & Learned & \multicolumn{4}{c}{Observations} \\
    \midrule
    & & & 10 & 30 & 50  & 100 \\
      \midrule
    \model &  \textbf{+} & \textbf{+} & \textbf{0.235 (0.001)}  & \textbf{0.162 (0.001)} & \textbf{0.146 (0.001)} & \textbf{0.121 (0.001)} \\
     Set Transformer  & \textbf{+}  & \textbf{+} &  0.390 (0.002) & 0.388 (0.002) & 0.388 (0.002) & 0.389 (0.001)\\
     LSTM & \textbf{+}  & \textbf{+} & 0.288 (0.001) & 0.260 (0.001) & 0.269 (0.001) & 0.288 (0.001) \\
     VQ  & \textbf{+}  & \textbf{-} & 0.246 (0.001) & 0.172 (0.001) & 0.147 (0.001)& 0.122 (0.001)\\
    \midrule
    Set Transformer & \textbf{-} &  \textbf{+} &  0.295 (0.003) & 0.261 (0.001) & 0.253 (0.001) & 0.247 (0.001)\\
     K-means++ & \textbf{-} &   \textbf{-} & \textbf{0.183 (0.002)} & \textbf{0.107 (0.001)} & \textbf{0.086 (0.001)} & \textbf{0.066 (0.001) }\\
     GMM & \textbf{-} & \textbf{-} & 0.189 (0.002) & 0.118 (0.001) & 0.087 (0.001) & 0.067 (0.001) \\
        \bottomrule
\end{tabular}
}
\caption{\small \textbf{Performance with Observation Number.} Comparison of performance after training on one thousand {\em Normal} distributions for a thousand iterations. We use 3 components, and train models with 30 observations. We report standard error in parentheses. Each cluster observation and center is drawn between -1 and 1, with reported error as the L2 distance between predicted and ground truth mean.}
\label{tbl:comparisons-normal}
\vspace{-15pt}
\end{table}




==> figText/illustration.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{fig/illustration2.pdf}
\vspace{-10pt}
\caption{\small \textbf{Qualitative Visualization of Domains.} Visualizations of the Normal Gaussian, Dynamic domains and Simulated Household domains. Observations are transparent while ground truth states are bolded for gaussian and dynamic domains. Four sample image observations shown for the simulated household robotic domain.}
\label{fig:illustration}
\vspace{-15pt}
\end{figure}


==> figText/main_tbl_full.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{5.5pt}
\centering

\begin{tabular}{l|c|c|cccc}
    \toprule
    Type & Model & Online & \multicolumn{4}{c}{Observations} \\
    \midrule
      & & & 10 & 30 & 50  & 100 \\
      \midrule
    \multirow{7}{*}{Normal} &  \model &  \textbf{+} & 0.235 & 0.162 & 0.146 & 0.128 \\
    & Set Transformer  & \textbf{+} & 0.390 & 0.388 & 0.388  & 0.389 \\
    & LSTM & \textbf{+} & 0.288  & 0.260  & 0.269  & 0.288  \\
    & VQ  & \textbf{+} & 0.246  & 0.172  & 0.147 & 0.122  \\
    & Set Transformer & \textbf{+} & 0.295  & 0.261  & 0.253  & 0.247  \\
    & K-means++ & \textbf{-} & 0.183  & 0.107 & 0.086 & 0.066    \\
    & GMM & \textbf{-} & 0.189  & 0.118 & 0.087  & 0.067  \\
    \midrule
    \multirow{7}{*}{Mixed} &  \model &  \textbf{+} & 0.255  & 0.184  & 0.164  & 0.147  \\
    & LSTM  & \textbf{+} &  0.306  & 0.274  & 0.284  & 0.290 \\
    & Set Transformer  & \textbf{+} & 0.415  &  0.405  & 0.407 & 0.408  \\
    & VQ & \textbf{+} & 0.262  & 0.192  & 0.169 & 0.145 \\
    & Set Transformer & \textbf{-} & 0.309 & 0.274  & 0.266   & 0.261  \\
    & K-means++ &  \textbf{-}& 0.206  & 0.135  & 0.105 & 0.088   \\
    & GMM & \textbf{-} &   0.212 & 0.136  & 0.105  & 0.079 \\
    \midrule
    \multirow{7}{*}{Enlongated} & \model & \textbf{+} &  0.258  & 0.192  & 0.173  & 0.161 \\
     & LSTM  & \textbf{+} &  0.314  & 0.274 & 0.288 & 0.300  \\
    & Set Transformer & \textbf{+} & 0.394 & 0.391  & 0.394  & 0.394  \\
    & VQ  & \textbf{+} & 0.265  & 0.194  & 0.172  & 0.149 \\
    & Set Transformer & \textbf{-} & 0.309 & 0.244 & 0.240  & 0.232 \\
      & K-means++  & \textbf{-} & 0.213  & 0.139  & 0.113  & 0.092  \\
     & GMM  & \textbf{-} & 0.214  & 0.141 & 0.112  & 0.086 \\
    \midrule
    \multirow{7}{*}{Rotation}  &  \model & \textbf{+} &  0.892  & 0.794  & 0.749  & 0.736  \\
      & LSTM & \textbf{+} & 0.799  & 0.796  & 0.795 & 0.794 \\
      & Set Transformer &  \textbf{+} & 0.793 & 0.794  & 0.782 & 0.782\\
      & VQ  & \textbf{+} & 0.956 & 1.000 & 1.000  & 0.984  \\
      & Set Transformer  & \textbf{-} &  0.815 & 0.784 &  0.779  & 0.772 \\
      & K-means++   & \textbf{-} & 0.827  & 0.834  & 0.823  & 0.802  \\
     & GMM & \textbf{-} & 0.842  & 0.875  & 0.867 & 0.848  \\
     \midrule
    \multirow{7}{*}{Noise}  & \model & \textbf{+} &  0.375  & 0.343 & 0.338 & 0.334  \\
     & LSTM & \textbf{+} &  0.419 & 0.406  & 0.405 & 0.407  \\
     & Set Transformer &  \textbf{+} & 0.434   & 0.424 & 0.425  & 0.424 \\
     & VQ & \textbf{+} & 1.479 & 0.948  & 0.826  & 0.720 \\
     & Set Transformer & \textbf{-} & 0.436  & 0.407 & 0.398 & 0.394 \\
     & K-means++ & \textbf{-} & 1.836  & 1.271  & 1.091  & 0.913  \\
     & GMM & \textbf{-}  & 1.731 & 1.215  & 1.056  & 0.856 \\

     
    \bottomrule
\end{tabular}
\caption{\textbf{Generalization with Increased Observations.} Error of different models when executed \textit{at test time} on different number of observations across different distributions. We train models with 3 components and 30 observations. }
\label{table:main_tbl_full}
\end{table*}

==> figText/qualitative_combined.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{fig/mnist_qualitative.pdf}
\includegraphics[width=\linewidth]{fig/airplane_qualitative.pdf}
\vspace{-10pt}
\caption{\small \textbf{Qualitative Visualization of \model Execution on Images. } Qualitative visualization of two image-based association tasks (left: MNIST, right: airplanes).  At the top of each is an example training problem, illustrated by the true objects and an observation sequence.  Each of the next rows shows an example test problem, with the ground truth objects and decoded slot values.  The three highest-confidence hypotheses for each problem are highlighted in red, and correspond to ground-truth objects.
} 
\label{fig:qualitative}
\vspace{-15pt}
\end{figure}

==> figText/qualtitative_clustering.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.9\linewidth]{fig/cluster_qual_large2.pdf}
\caption{\small \textbf{Qualitative Visualization of \model.} Illustration of \model execution on the {\em Normal} distribution setting. Decoded value of hypothesis (with size corresponding to confidence) shown in red, with ground truth clusters in black. Observations are shown in blue. } 
\label{fig:qualitative_clustering}
\vspace{-5pt}
\end{figure*}

==> figText/update_weight_at_vis.tex <==


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{fig/at_map_vis_new.pdf}
    \caption{\small \textbf{Visualization of Attention Weights.} Plot of decoded values of slots (in red) with confidence shown by the size of dot (left), and what slot each input assigns the highest attention towards (right) (each slot is colored differently, with assigned inputs colored in the same way).  Note alignment of regions on the right with the decoded value of a slot on the left.}
    \label{fig:at_vis}
    \vspace{-10pt}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{fig/update_weight.pdf}
    \vspace{-5pt}
    \caption{\small \textbf{Visualization of Relevance Weights.} Plots of the magnitude of relevance weights with increased observation number on different distributions with differing standard deviation (noise).  }
    \label{fig:update_weight}
    \vspace{-15pt}
\end{figure}

==> new_figText/gen_hypothesis.tex <==
\begin{table}
    \centering
    \small
    \scalebox{0.8}{
    \begin{tabular}{l|c|ccc}
        \toprule
        Model &  Slots & \multicolumn{3}{c}{Ground Truth Clusters} \\
        \midrule
          & &  3 & 5 & 7 \\
         \midrule
        \multirow{3}{*}{\model} & 10 & \textbf{0.162} & 0.214 & 0.242 \\
          &  20 & 0.175  & \textbf{0.195} & 0.213 \\
         &  30 &  0.188  & 0.197  & \textbf{0.205}\\
         \midrule
        Set Transformer & - & 0.261 & 0.279  & 0.282  \\
        \midrule
        Vector Quantization & - & 0.171  & 0.199  & \textbf{0.205} \\
         \bottomrule
    \end{tabular}
    }
\caption{\small \textbf{Generalization with Different Hypothesis Slots.} 
Error of \model , when executed {\em at test time} with a different number of hypothesis slots on test distributions with different numbers of ground true components. In all cases, \model is trained on 3-component problems with 10 slots. \model achieves good performance with novel number of hypothesis slots, and outperforms different instances of the Set Transformer trained with the ground truth number of cluster components as well as vector quantization.}
\label{tbl:hypothesis_gen}
\vspace{-15pt}
\end{table}
